A Gaussian variational inference approach to motion planning

We propose a Gaussian variational inference framework for the motion planning problem. In this framework, motion planning is formulated as an optimization over the distribution of the trajectories to approximate the desired trajectory distribution by a tractable Gaussian distribution. Equivalently, the proposed framework can be viewed as a standard motion planning with an entropy regularization. Thus, the solution obtained is a transition from an optimal deterministic solution to a stochastic one, and the proposed framework can recover the deterministic solution by controlling the level of stochasticity. To solve this optimization, we adopt the natural gradient descent scheme. The sparsity structure of the proposed formulation induced by factorized objective functions is further leveraged to improve the scalability of the algorithm. We evaluate our method on several robot systems in simulated environments, and show that it achieves collision avoidance with smooth trajectories, and meanwhile brings robustness to the deterministic baseline results, especially in challenging environments and tasks.

==> gaussian_quadratures.tex <==
\section{Gauss-Hermite quadrature and the evaluation of the derivatives}
From  \ref{eq:deriv1_k} and  \ref{eq:deriv2_k} it is clear that the key to calculating the derivatives involves the evaluation of several expectations w.r.t. a Gaussian distribution $q_k$. Gauss-Hermite quadrature\cite{} is a numerical method used to approximate these expectation. To compute the integration of a scalar function $g(\bx)$ w.r.t. a Gaussian distribution
\begin{equation}
    \int g(\bx) \calN(\bx; \bm, \bP) d\bx,
    \label{eq:target_integration}
\end{equation}
Gauss-Hermite quadrature methods consist of
\begin{enumerate}
    \item Compute the $p$ roots of a $p\; th$ order Hermite polynomial, also denoted as sigma points
    \begin{equation}
        \bxi = [\bxi_1, \dots, \bxi_p].
    \end{equation}
    \item Compute the weights
    \begin{equation}
        W_i = \frac{p!}{p^2[H_{p-1}(\bxi_i)]}, i=1, \dots, p.
    \end{equation}
    \item Approximate the integral \ref{eq:target_integration}
    \begin{equation}
        \int g(\bx) \calN(\bx;\bm,\bP) d\bx \approx \sum_{l=1}^{p^n} \Tilde{W}_l g(\sqrt{\bP}\Tilde{\bxi}_l + \bm),
    \end{equation}
    where $\Tilde{\bxi}_l$ is a $n$ dimensional vector which is the concatenation of a permutation of the sigma points, i.e., $\Tilde{\bxi_l} = [\bxi_{l_1}, \dots, \bxi_{l_n}]$, and $l_1, \dots, l_n \in [1, \dots, p]$, and $\Tilde{W}_l$ is the the product of all the corresponding weights, i.e., $\Tilde{W}_l = \prod_{i=1}^{n}W_{l_i}$.
\end{enumerate}
It is straightforward to see that for an approximation of a $n$-dimensional integration, $p^n$ sigma points are needed, which is computationally costly in high dimensional problems. In our  robotics problems, the integrations are carried out on the factor level, which mitigates this issue.   



==> sparse_inverse.tex <==
\subsection{Computing the marginal covariance}
{\chen discuss several approaches. remark}
While the joint precision matrix remains sparse throughout the iterations, the covariance matrix need not to be sparse. However, for a matrix with known sparsity pattern, methods exist in the sparse linear algebra community \cite{} to efficiently compute its inverse. For a sparse matrix $\bY$, first we conduct an $LDL^T$ decomposition $\bY = \bL\bD\bL^T$, where $\bL$ is a lower-triangular matrix with ones on diagonals, and $\bD$ is diagonal. The sparsity pattern of matrix $\bL$ is related to the sparsity pattern of $\bY$. We then have 
\begin{equation}
    \bL\bD\bL^T\bY^{-1} = \bI
\end{equation}
where $\bI$ is the identity matrix. Multiply the two sides from left by the inverse of $\bL\bD$, we arrive at
\begin{equation}
    \bL^T\bY^{-1} = \bD^{-1}\bL^{-1}.
\end{equation}
Take the transpose and add $\bY^{-1} - \bY^{-1} \bL$ to both sides, and we arrive at
\begin{equation}
    \bY^{-1} = \bL^{-T}\bD^{-1} + \bY^{-1}(\bI - \bL).
    \label{eq:iterative_bsigma}
\end{equation}
$\bL^T$ is upper-triangular with ones on the diagonal, and $\bI-\bL$ has zeros on its diagonal. From \eqref{eq:iterative_bsigma} we start the iterative calculations of $\bY^{-1}$. We calculate only the lower-triangular part of the symmetric $\bY^{-1}\in \mR^{T\times T}$. Starting from
\begin{equation}
    \bY^{-1}_{T,T} = \frac{1}{\bD_{T,T}},
    \label{eq:Sigma_KK}
\end{equation}
the calculation traces back as
\begin{equation}
\begin{split}
    \bY^{-1}_{T, T-1} &= -\bL_{T, T-1}\bY^{-1}_{T,T}, \\
    \bY^{-1}_{T-1, T-1} &= \frac{1}{\bD_{T-1,T-1}},\\
    \bY^{-1}_{T, T-2} &= -\bL_{T,T-2}\bY^{-1}_{T,T} - \bL_{T-1, T-2}\bY^{-1}_{T,T-1},\\
    &\dots \\
    \bY^{-1}_{i, j} &= \begin{cases}
      \bD^{-1}_{i,i}, & \text{if}\ i=j \\
      -\sum_{m=j+1}^{T}\bY^{-1}_{i, m} \bL_{m, j}, & \text{otherwise.}
    \end{cases}
\end{split}
\label{eq:Sigma_iter}
\end{equation}
The matrix $\bL$ is sparse and its pattern can be known from  $\bY$ by the rule of 'four corners of a box' \cite{barfoot2020exactly}\cite{erisman1975computing}. Fig. \ref{fig:sparse} shows the sparsity pattern of $\bSigma^{-1}$ and $\bL$ for a planar point robot. The sparsity pattern encodes the Markov property of the Gaussian process motion planning \cite{barfoot2014batch}. 

\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figures/planar_pR/sparse.eps}
    \caption{Typical sparsity pattern for $\bSigma^{-1}$ and $\bL$.}
    \label{fig:sparse}
\end{figure}

We summarize the main algorithm in this paper in Algorithm \ref{algo:GVIMP}.
\begin{algorithm}[!ht]
\DontPrintSemicolon
  \KwInput{$\bmu, \bSigma^{-1}, \textrm{SDF}, \{\bP_k\}_{k=1}^N$, \textrm{threshold} $\eta$}
  \KwOutput{$\bmu, \bSigma^{-1}$} 
  {\chen loop?}
  \While {true}{
    Compute $\bSigma$ using \eqref{eq:Sigma_KK} and \eqref{eq:Sigma_iter}\\
      Compute $\bmu_k, \bSigma_k$ using \eqref{eq:transform_factor}\\
      Update $\bmu_k, \bSigma^{-1}_k$ using \eqref{eq:derivs_k}, the expectations are computed using Gauss-Hermite quadratures. The prior is computed on a factorized level using \eqref{eq:prior_factors} and the costs are computed also on a factorized level using SDF.\\
      Compute $\frac{\partial V(q)}{\partial \bmu}, \frac{\partial^2 V_k(q_k)}{\partial \bmu_{k}\bmu_{k}^T}$ using \eqref{eq:derivs}\\
      Compute $\bmu, \bSigma^{-1}$ using \eqref{eq:fact_update}\\
      Compute $\delta \bSigma^{-1}$ using \eqref{eq:deltaSigma} and compute $\delta \bmu$ by solving the first equation in \eqref{eq:ngd_step}\\
      Do the backtracking using \eqref{eq:backtracking} to update $\bmu, \bSigma^{-1}$.
      
      \If {Objective \eqref{eq:factorized_obj} decreases less than $\eta$}
      {Break.}
  }
  
\caption{Gaussian VI motion planning}
\label{algo:GVIMP}
\end{algorithm}

% {\chen summarize our algorithm}

